Estimating Entropy of Distributions in Constant Space

We consider the task of estimating the entropy of $k$-ary distributions from samples in the streaming model, where space is limited. Our main contribution is an algorithm that requires $O\left(\frac{k \log (1/\varepsilon)^2}{\varepsilon^3}\right)$ samples and a constant $O(1)$ memory words of space and outputs a $\pm\varepsilon$ estimate of $H(p)$. Without space limitations, the sample complexity has been established as $S(k,\varepsilon)=\Theta\left(\frac k{\varepsilon\log k}+\frac{\log^2 k}{\varepsilon^2}\right)$, which is sub-linear in the domain size $k$, and the current algorithms that achieve optimal sample complexity also require nearly-linear space in $k$. Our algorithm partitions $[0,1]$ into intervals and estimates the entropy contribution of probability values in each interval. The intervals are designed to trade off the bias and variance of these estimates.

==> app-general-algorithms.tex <==
We provide the pseudocode of the various procedures for our main algorithms in this section. 

Algorithm~\ref{alg:interval-general} is the interval estimation algorithm that tests from samples where a $p(x)$ belongs to a certain interval $I_t$. 

\begin{algorithm}[h]
		\caption{Estimating intervals: General Case : \textsc{GenEstInt}$(\bset{t},x)$} \label{alg:interval-general}
		\begin{algorithmic}[1]
			\Require $\bset{t},x$ drawn from $p$
			\For{$i = 1 \text{ to } t  $}
			\State Generate $\bSmp_i$ samples from $p$ 
			\State {\textbf{if} $x$ appears more than $\bSmp_i \ell_i$ times  \textbf{then} Output $I_i$}
			\EndFor
			%\State Generate $\bSmp_t$ samples from $p$ 
			%\State {\textbf{if} $x$ appears more than $\bSmp_t \ell_t$ times \textbf{then} Output $I_t$}
			%\State{\textbf{else} Output $I_T$}
			\State Output $I_T$
		\end{algorithmic}
	\end{algorithm} 


Algorithm~\ref{alg:estp_general} describes the procedure to estimate $\p_\cA(I_t)$'s. 
\begin{algorithm}[h]
 	\caption{Estimating $p_\cA\left(I_i \right),1 \leq i \leq T-1$ : \textsc{GenEstProbInt}$(\bset{T-1},\vset{T-1})$ } \label{alg:estp_general}
 	\begin{algorithmic}[1]
 	\Require $\bset{T-1},\vset{T-1}$
 		\For{$i = 1, 2, ..., T-1$}
 		\State $\hat{p}_\cA\left(I_i\right) = 0$
 		\For{$t = 1 \text{ to } \vSmp_i$}
 		\State Sample $x \sim \p$.
 		\State{\textbf{if} $\textsc{GenEstInt}\left(\left \lbrace \bSmp_j \right \rbrace_{j = 1}^{i} , x\right) = I_i$ \textbf{then} $\hat{p}_\cA\left(I_i \right)= \hat{p}_\cA\left(I_i \right)+ \frac{1}{\vSmp_i}$}	
 		\EndFor
 		\EndFor
 		%$\hat{p}_{\cA} \left(I_T\right) = 1 - \sum\limits_{i=1}^{T-1} 	\hat{p}_{\cA} \left(I_i\right)$
 	\end{algorithmic}
 \end{algorithm} 

Algorithm~\ref{alg:esth_general} estimates the entropy contributions from the intervals. 
\begin{algorithm}[h]
	\caption{Estimating ${H}_i$'s : \textsc{GenCondExp}$\left( \bset{T}, \vset{T} \right)$} \label{alg:esth_general}
	\begin{algorithmic}[1]
	\Require $\bset{T},\vset{T}$
		\For{$i=1 \text{ to } T$}
		\State $\hat{H}_i = 0, S_i = 0$
		\For{$t = 1 \text{ to } \vSmp_i$}
		\State Generate $x \sim p$
		\If{$\textsc{GenEstInt}\left(\left \lbrace \bSmp_j \right \rbrace_{j = 1}^{i}, x\right)$is $I_i$}
		\State $S_i = S_i + 1$
		\State Let $N_{x,i} \leftarrow$ \# occurrences of $x$  in the next $\bSmp_i$ samples
		\State $E_{x,i} = \max \{ \log \left(\frac{\bSmp_i}{N_{x,i} + 1} \right), \log \frac{1}{4h_i}\} $ \label{clipping_gen}
		\State $\hat{H}_i = \hat{H}_i +E_{x,i} $ 
		\EndIf
		\EndFor
		\State $\bar{H}_i = \frac{\hat{H}_i}{S_i}$
		\EndFor
		%	\State Output  $\hat{H} = \sum_{i = 1}^{T - 1}\hat{p}\left[I_i\right] \hat{H_i} + \left(1-\sum_{i = 1}^{T - 1} \hat{p}\left[I_i\right]\right) \hat{H_T}$
	\end{algorithmic}
\end{algorithm} 


==> app-memory-requirements.tex <==
%\section{Memory Requirements of Algorithms}\label{sec:memory}
%In this section we explicitly count the memory requirements of the algorithms in Section~\ref{sec:interval} and ~\ref{sec:simplealgo}

%\noindent\textbf{Memory Requirements of Algorithm~\ref{alg1}.}
%\newer{We  reserve two words for $\bSmp$, $\vSmp$. We reserve one word each to store $S,x$ and each of the $N$ symbols. We reserve two words for $N_x$ and three words for the counters. Thus the algorithm uses less than 20 words of space.}

%\medskip
%\noindent \textbf{Memory Requirements for Algorithm~\ref{alg:twoint}.} 
%For all parameters on Line~\ref{step:params}, we reserve two words and compute them on the fly. It is sufficient to use two words to store one of $\hat{p}_{\cA}\left(I_1\right)$ and $\hat{p}_{\cA}\left(I_2\right)$, and one of $\hat{H}_1$ and $\hat{H}_2$ since both $\textsc{EstProbInt}$ and $\textsc{CondExp}$ can be executed for each interval together. We use one word to store the final estimate $\estII$. \textsc{EstInt} uses one word each to store $x$, a symbol of the stream of $\bSmp$ samples, the interval, and to count occurrences of $x$. \textsc{CondExp} requires four more words to store $i,S_i,N_i,N_{x,i}$. None of the algorithms require more than three counters at once for which we use four words in total. Hence, at most 20 words of memory are required.
%One word each is required to store $\ell, \bSmp_1, \bSmp_2, \vSmp_1, \vSmp_2$. One word each is required to store $\bar{H}_1, \bar{H}_2,  \hat{p}_\cA\left(I_1 \right), \hat{p}_\cA\left(I_2 \right)$ and $\estII$. \textsc{EstProbInt} requires one word to store the counter of the for loop, three words for \textsc{EstInt} and one word for the output of \textsc{EstInt}. Note that once \textsc{EstProbInt} is executed, these words can be freed up for subsequent usage. \textsc{CondExp} uses two words to store $\hat{H}_i, S_i$ and one word to store $i$. The words freed up after executing  \textsc{EstProbInt} can be used again for the same purpose in \textsc{CondExp}. Finally, one more word is used to store $N_{x,i}$. Therefore, Algorithm~\ref{alg:twoint} uses atmost 20 words.

%\medskip 
%\noindent\textbf{Memory Requirements of Algorithm~\ref{alg:genint}}
%We reserve one word to compute $\hat{p}_{\cA} \left(I_T\right)$. Apart from this, we require the same memory as that of the two interval algorithm since \textsc{GenEstInt}, \textsc{GenEstProbInt} and \textsc{GenCondExp} require same memory as that of their two interval counterparts. Also, we perform one iteration each of \textsc{GenEstProbInt} and \textsc{GenCondExp} and maintain running sum of $\hat{p}_{\cA} \left(I_i\right) \bar{H}_i$'s. Therefore, Algorithm~\ref{alg:genint} requires at most 20 words of space.




==> app-preliminaries.tex <==



==> mdlintvlpf.tex <==
\subsection{Proof of Lemma~\ref{lem:mdlbias} : Bias Bound}
From Algorithm~\ref{alg1}, we can express $\bar{H}$ as 
 \begin{align*}
 \bar{H} &= \frac{1}{\vSmp}\sum\limits_{t=1}^{\vSmp} \sum\limits_{x\in \mathcal{X}} \indctr{ x = x_t }\log \left( \frac{\bSmp}{N_{x_t} + 1} \right). \\
 &=  \sum\limits_{x\in \mathcal{X}} \frac{1}{\vSmp}\sum\limits_{t=1}^{\vSmp} \indctr{ x = x_t }\log \left( \frac{\bSmp}{N_{x_t} + 1} \right).
 \end{align*}
 The above formulation can be thought of as an empirical average of $\log\left( \frac{\bSmp}{N_X+1} \right)$, where $X \sim p$. 
Therefore, 

\begin{equation}
\Expc{\bar{H}} =\sum\limits_{x \in \mathcal{X}} p\left( x \right) \Expc{ \log \left( \frac{\bSmp}{N_{x}+1} \right)}.
\end{equation}

 
 
% Therefore,
%\begin{align*}
%\Expc{\bar{H}} &=\frac{1}{\vSmp} \sum\limits_{t=1}^{\vSmp} \sum\limits_{x \in \mathcal{X}} \Expc{ \indctr{x = x_t} \log \left( \frac{\bSmp}{N_{x_t}+1} \right) }\\
%&= \frac{1}{\vSmp} \sum\limits_{t=1}^{\vSmp} \sum\limits_{x \in \mathcal{X}} p\left(x\right) \Expc{ \log \left( \frac{\bSmp}{N_{x_t}+1} \right) \mid x_t = x }.
%\end{align*} 
%Note that, given $x_t = x$, $N_{x_t} \sim \text{Bin} \left(\bSmp,p\left(x\right) \right)$. We drop the conditional expectation and denote $N_{x_t}$ as $N_{x,x_t}$ from now.
%\begin{equation*}
%\Expc{\bar{H}} =\frac{1}{\vSmp} \sum\limits_{t=1}^{\vSmp} \sum\limits_{x \in \mathcal{X}} p\left(x\right)\Expc{ \log \left( \frac{\bSmp}{N_{x,x_t} + 1} \right)}.
%\end{equation*}

\begin{align}
\Ent{p} -  \Expc{ \bar{H}} &= \sum\limits_{x \in \mathcal{X}} p\left(x\right) \log \frac{1}{p\left(x\right)} - \sum\limits_{x\in \mathcal{X}} p\left(x\right)\Expc{\log \left( \frac{\bSmp}{N_{x}+1} \right)} \nonumber \\
&= \sum\limits_{x \in \mathcal{X}} p\left(x \right) \Expc{ \log \left( \frac{N_{x}+1}{\bSmp p\left(x\right)} \right)}  \nonumber \\
&\leq \sum\limits_{x \in \mathcal{X}} p\left(x \right)  \log \left( \Expc{\frac{N_{x}+1}{\bSmp p\left(x\right)}}  \right) \label{eq:modelJens} \\
&= \sum\limits_{x \in \mathcal{X}} p\left(x \right)  \log \left( 1 + \frac{1}{\bSmp p\left(x\right)} \right) \nonumber \\
&\leq \frac{k}{\bSmp}. \label{eq:logineq}
\end{align}
where we obtain \eqref{eq:modelJens} using Jensen's inequality and \eqref{eq:logineq} follows from $\log \left(1+x \right) \leq x$. We now bound $\Expc{\bar{H}} - \Ent{p}$.

\begin{align}
\Expc{\bar{H}} - \Ent{p} &= \sum\limits_{x \in \mathcal{X}} p\left(x \right) \Expc{\log \left( \frac{\bSmp p\left(x\right)}{N_{x}+1} \right)} \nonumber \\
&\leq \sum\limits_{x \in \mathcal{X}} p\left(x \right)  \log \left( \Expc{\frac{\bSmp p\left(x\right)}{N_{x}+1}} \right) \label{eq:mdlJens}\\
&\leq  \sum\limits_{x \in \mathcal{X}} p\left(x \right) \log \left( \frac{\bSmp}{\bSmp+1} \right) < 0. \label{eq:invbinom}
\end{align}
where \eqref{eq:mdlJens} is obtained using Jensen's inequality and \eqref{eq:invbinom} follows from  Lemma~\ref{binreciplemma}. Therefore,
\begin{equation} \label{bias}
\lvert \Expc{\bar{H}} - \Ent{p} \rvert \leq \dfrac{k}{\bSmp} .
\end{equation} 


==> one-interval__Sourbh_Bhadane_s_conflicted_copy_2019-11-12_.tex <==
%The key idea in the \naive algorithm is to estimate $\log\left(p \left(x\right) \right)$ independent of $p\left(x\right)

\section{A Building Block: Simple Algorithm with Constant Space}\label{sec:simplealgo}

%The idea behind the model algorithm is based on the following observation:
%	\[
%	H(p) = \EE_{X \sim p} [\log \frac{1}{p(X)}]
%\]
We propose a simple method (Algorithm~\ref{alg1}) with the following guarantee. 
%\vspace{-5pt}
\begin{theorem}
\label{thm:one-interval}
Let $\eps>0$. Algorithm~\ref{alg1} takes $O\left(\frac{k\log^2 \left(k/\eps\right)}{\eps^3}\right)$ samples from $\p\in\Delta_k$, uses at most 20 words of memory, and outputs $\bar H$, such that with probability at least $2/3$, $\abs{\bar H - H(\p)}<\eps$.
\end{theorem}

%Algorithm~\ref{alg1} elaborates the two steps described in the beginning of Section~\ref{sec:techniques} by specifying precise values of $N$ and $R$ needed to bound the bias and concentration. The basis of the approach is from~\eqref{eqn:expansion-entropy}. 

Based on ~\eqref{eqn:expansion-entropy}, each iteration of Algorithm~\ref{alg1} obtains a draw $X$ from $\p$ and estimates $\log(1/\p(X))$. To avoid assigning zero probability value to $\p(X)$, we do add-1 smoothing to our empirical estimate of $\p(X)$. The bias in our estimator can be controlled by the choice of $N$. %The final estimator is the empirical mean of $R$ independent estimates $\widehat H_1 \ldots \widehat H_R$.
\begin{algorithm}[ht]
	\caption{Entropy estimation with constant space: Simple Algorithm} \label{alg1}
	\begin{algorithmic}[1]
	\Require Accuracy parameter $\eps>0$, a data stream $X_1, X_2, \ldots\sim p$
		\State Set 
		%\vspace{-10pt}
%		\[
%		R \gets \frac{4\log^2(1+2k/\eps)}{\eps^2},\qquad \bSmp \gets \frac{2k}{\eps}, \qquad S \gets 0
%		\]
		\[
			R \gets 4\log^2(1+2k/\eps)/\eps^2,\qquad \bSmp \gets 2k/\eps, \qquad S \gets 0
		\]
		%\vspace{-20pt}
		\For{$t=1, \ldots, \vSmp $}
		\State Let $x\gets$ the next element in the data stream 
		\State $N_{x}\gets$ \# appearances of $x$ in the next $\bSmp$ symbols
		%\State $\widehat{H}_t = \log\left(\frac{\bSmp}{N_{x} + 1}	\right) $
		\State $\widehat{H}_t = \log\left({\bSmp}/({N_{x} + 1})	\right) $		 \label{entstepalg1}
		\State  $S = S + \widehat{H}_t$
		\EndFor
		\State $\bar{H} = S/ \vSmp$
	\end{algorithmic}
\end{algorithm}

%Algorithm~\ref{alg1}  We explicitly count these in .
%\medskip
%\noindent\textbf{Memory Requirements of Algorithm~\ref{alg1}.}
%\newer{We  reserve two words for $\bSmp$, $\vSmp$. We reserve one word each to store $S,x$ and each of the $N$ symbols. We reserve two words for $N_x$ and three words for the counters. Thus the algorithm uses less than 20 words of space.}
%\anote{Show that the algorithm needs at most 10 words of space?}
\noindent\textbf{Performance Guarantee.}
%Algorithm~\ref{alg1} only maintains a running sum at the end of each iteration can be implemented with 20 words of space (Section~\ref{sec:memory}). To bound the accuracy, note that $\bar H$ is the mean of $R$ i.i.d. random variables $\widehat H_1, \ldots, \widehat H_R$. We bound the bias and prove concentration of $\bar H$ using Lemma~\ref{lem:hoeff}.

%Algorithm~\ref{alg1} only maintains a running sum at the end of each iteration. We reserve two words for $\bSmp$, $\vSmp$ and $S$ each. We reserve one word to store $x$ and two words to keep track of $N_x$ in each iteration. We reserve three words for the counters. Thus the algorithm uses less than 20 words of space.

Algorithm~\ref{alg1} only maintains a running sum at the end of each iteration. Since $\bSmp, \vSmp$ are program constants they are computed on the fly. We reserve one word to store $x$ and two words to keep track of $N_x$ in each iteration. We reserve in total, four words for the counters and two words to store $S$ (and the final entropy estimate). Thus the algorithm uses less than 20 words of space.

 To bound the accuracy, note that $\bar H$ is the mean of $R$ i.i.d. random variables $\widehat H_1, \ldots, \widehat H_R$. We bound the bias and prove concentration of $\bar H$ using Lemma~\ref{lem:hoeff}.

%\medskip
\noindent\textit{Bias Bound.} Large $N$ in Algorithm~\ref{alg1} gives a better estimate of $\p(X)$, and small bias in entropy estimation.
\begin{lemma}(\textbf{Bias Bound})\label{lem:mdlbias}
	%\begin{equation}
	$\left \lvert \Expc{\bar{H}}-\Ent{p}  \right \rvert \leq \frac{k}{\bSmp}. \nonumber$
	%\end{equation}
\end{lemma}
\begin{proof}
Each iteration of Algorithm~\ref{alg1} chooses $x$ drawn from $p$. Therefore, 
%From Algorithm~\ref{alg1}, we can express $\bar{H}$ as 
% \begin{align*}
% \bar{H} &= \frac{1}{\vSmp}\sum\limits_{t=1}^{\vSmp} \sum\limits_{x\in \mathcal{X}} \indctr{ x = x_t }\log \left( \frac{\bSmp}{N_{x_t} + 1} \right). \\
% &=  \sum\limits_{x\in \mathcal{X}} \frac{1}{\vSmp}\sum\limits_{t=1}^{\vSmp} \indctr{ x = x_t }\log \left( \frac{\bSmp}{N_{x_t} + 1} \right).
% \end{align*}
% The above formulation can be thought of as an empirical average of $\log\left( \frac{\bSmp}{N_X+1} \right)$, where $X \sim p$. 
%Therefore, 
\begin{equation}
\Expc{\bar{H}} =\Expc{\bar{H}_t}=\sum\limits_{x \in [k]} p\left( x \right) \Expc{ \log \left( \frac{\bSmp}{N_{x}+1} \right)},
\end{equation}
where the expectation is over the randomness in $N_x$. 
Therefore, 
\begin{align}
\Ent{p} -  \Expc{ \bar{H}} = \sum\limits_{x \in [k]} p\left(x\right) \log \frac{1}{p\left(x\right)} - \sum\limits_{x\in [k]} p\left(x\right)\Expc{\log \left( \frac{\bSmp}{N_{x}+1} \right)}
= \sum\limits_{x \in [k]} p\left(x \right) \Expc{ \log \left( \frac{N_{x}+1}{\bSmp p\left(x\right)} \right)}.  \nonumber
\end{align}
We now bound this expression. 
\begin{align}
 \sum\limits_{x \in [k]} p\left(x \right) \Expc{ \log \left( \frac{N_{x}+1}{\bSmp p\left(x\right)} \right)}
\stackrel{(a)}{\leq} \sum\limits_{x \in [k]} p\left(x \right)  \log \left( \Expc{\frac{N_{x}+1}{\bSmp p\left(x\right)}}  \right) 
\stackrel{(b)}{=} \sum\limits_{x \in [k]} p\left(x \right)  \log \left( 1 + \frac{1}{\bSmp p\left(x\right)} \right)
\stackrel{(c)}{\leq} \frac{k}{\bSmp},\nonumber
\end{align}
where $(a)$ uses concavity of logarithms, $(b)$ follows since $N_x$ is distributed $Bin(N, p(x))$ and therefore has mean $N p(x)$, and $(c)$ uses $\log (1+x)\le x$. To lower bound the expression, we upper bound its negative. 
%\begin{align}
%\Ent{p} -  \Expc{ \bar{H}} &= \sum\limits_{x \in \mathcal{X}} p\left(x\right) \log \frac{1}{p\left(x\right)} - \sum\limits_{x\in \mathcal{X}} p\left(x\right)\Expc{\log \left( \frac{\bSmp}{N_{x}+1} \right)} \nonumber \\
%&= \sum\limits_{x \in \mathcal{X}} p\left(x \right) \Expc{ \log \left( \frac{N_{x}+1}{\bSmp p\left(x\right)} \right)}  \nonumber \\
%&\leq \sum\limits_{x \in \mathcal{X}} p\left(x \right)  \log \left( \Expc{\frac{N_{x}+1}{\bSmp p\left(x\right)}}  \right) \label{eq:modelJens} \\
%&= \sum\limits_{x \in \mathcal{X}} p\left(x \right)  \log \left( 1 + \frac{1}{\bSmp p\left(x\right)} \right) \nonumber \\
%&\leq \frac{k}{\bSmp}. \label{eq:logineq}
%\end{align}
\begin{align}
\sum\limits_{x \in [k]} p\left(x \right) \Expc{\log \left( \frac{\bSmp p\left(x\right)}{N_{x}+1} \right)}
&\stackrel{(a)}{\leq} \sum\limits_{x \in \mathcal{X}} p\left(x \right)  \log \left( \Expc{\frac{\bSmp p\left(x\right)}{N_{x}+1}} \right) 
\stackrel{(b)}{\leq}  \sum\limits_{x \in \mathcal{X}} p\left(x \right) \log \left( \frac{\bSmp}{\bSmp+1} \right) < 0. \label{eq:invbinom}
\end{align}
where $(a)$ uses concavity of logarithms and \eqref{eq:invbinom} follows from the following claim plugging in $r=p(x)$, and $m=N$. 

\begin{lemma}\label{binreciplemma}
Let $X \sim \text{Bin} \left(m,r\right)$, then
$
\Expc{\frac{1}{X+1}} \leq \frac{1}{r\left(m+1\right)}.
$%\end{equation*}
\end{lemma}
%\begin{proof}
%\vspace{-\topsep}
\begin{proof}
\[
	\Expc{\frac{1}{X+1}} = \frac1{m+1}\sum\limits_{l=0}^{m} \frac{m+1}{l+1} {{m}\choose{l}} r^l\left(1-r\right)^{m-l}= \frac{1-(1-r)^{m+1}}{r\left(m+1\right)}\leq \frac{1}{r\left(m+1\right)}.\qedhere
\]
\end{proof}
\noindent Combining the upper and lower bound on $\Ent{p} -  \Expc{ \bar{H}}$ proves the lemma.
\end{proof}

%\medskip
\noindent\textit{Concentration.} Using Hoeffding's inequality, we prove the following concentration result for $\widehat{H}$.
\begin{lemma}(\textbf{Concentration})
\label{lem:concentration-simple}
For any $\mu>0$,
$ \label{eqn:cnvrge}
\Pr \left( \lvert \bar{H} - \Expc{\bar{H}} \rvert \geq \mu \right) \leq 2\exp \left(- \frac{2R\mu^2}{\log^2 \left(\bSmp+1\right)} \right).$
\end{lemma}
\begin{proof}
In each of the $R$ iterations, $N_x$ takes a value in $\{0, \ldots, N\}$. Therefore, for $t=1, \ldots, R$, $\widehat{H}_t\in[\log (N/(N+1)), \log N]$ are i.i.d. random variables. 
%Note that $\bar{H}$ is an average of $\vSmp$ i.i.d random variables $$Z_t = \sum\limits_{x \in \mathcal{X}} \indctr{x=x_t} \log \left( \frac{\bSmp}{N_{x_t} + 1} \right).  $$ where $t \in \range{\vSmp}$. Each of the $\vSmp$ random variables can take values from $ \range[\log \left( \frac{\bSmp}{\bSmp+1}\right)]{\log \bSmp}$. 
By Hoeffding's inequality (Lemma~\ref{lem:hoeff}), 
\begin{equation} \label{cnvrge}
\Pr \left( \lvert \bar{H} - \Expc{\bar{H}} \rvert \geq \frac{\eps}{2} \right) \leq \exp \left(- \frac{\vSmp \eps^2}{2\log^2 \left(\bSmp+1\right)} \right).\qedhere
\end{equation} 
\end{proof}
%With these two lemmas, we can conclude the sample complexity bounds as follows. 
The choice of $\bSmp$ in Algorithm~\ref{alg1} implies that $\left \lvert \Expc{\bar{H}}-\Ent{p}  \right \rvert \le\eps/2$, and by choosing  $\mu=\eps/2$, and $R =  {4\log^2(1+2k/\eps)}/{\eps^2} $ implies that $\bar H$ is within $H(\p)\pm\eps/2$ with probability at least $2/3$. This gives the total sample complexity of $(\bSmp+1) \vSmp = O\left({k\log^2 \left(k/\eps\right)}/{\eps^3}\right)$.

%From Lemma~\ref{lem:mdlbias} and~\ref{lem:concentration-simple}, notice that $\bSmp$ controls the bias and $\vSmp$ controls the concentration of the estimator. The key idea to reduce the sample complexity is the following observation: For symbols with large probability, we can make $\bSmp$ smaller since they are easy to estimate. For symbols with smaller probability, we can make $\vSmp$ smaller since its easier to control the variance because $\widehat{H}$'s will be in a smaller range with high probability. We formalize this notion in the next section. 





%%NOTE : The following is a comment 
\begin{comment} 
\scolor{Note that we use $\log\left(\dfrac{\bSmp}{N_{x_t} + 1} \right)$ instead of $\log\left(\dfrac{\bSmp}{N_{x_t}}\right) $ to avoid the case when $N_{x_t} = 0$. Since counting and cumulative sum can both be implemented using constant memory, so is this algorithm. Next we show how to choose $R$ and $n$ to satisfy the accuracy constraint.

Let $X \sim \p$ and define the following random variable:
\[
	\widehat{H} = \log\left(\dfrac{\bSmp}{N_{X} + 1}	\right)  = \sum\limits_{x \in \mathcal{X}} \indctr{X  = x} \log \left( \frac{n}{N_{x} + 1} \right) 
\] 
where $N_x$ is the number of appearances of $x$ when we sample $n$ independent samples from $\p$. Then the output of Algorithm~\ref{alg1} is the average of $R$ independent samples of $\widehat{H}$. We observe that the absolute error can be bounded by the following two terms:
	
%be a random variable coming from the following two steps: i) sample $X$ from $p$; ii) sample $\bSmp$ more samples and $X$ appears $N_X$ times in it. Then we can see our output is the average of $R$ independent samples of $\widehat{H}$. We observe that the absolute error can be bounded by the following two terms:
\[
	 |\Ent{p} -  \bar{H} | \le | \Ent{p} -  \Expc{\widehat{H}} | + |\bar{H} -  \Expc{ \widehat{H}} |.
\]

The first term can be bounded via the following lemma:

For the second term, which is the concentration term, we observe that each of the $R$ random variables can  onlytake values from $ \range[\log \left( \frac{n}{n+1}\right)]{\log n}$. Applying Hoeffding's inequality, 
\begin{equation} \label{cnvrge}
\Pr \left( \lvert \bar{H} - \Expc{\widehat{H}} \rvert \leq \frac{\eps}{2} \right) \leq 2\exp \left(- \frac{R\eps^2}{2\log^2 \left(n+1\right)} \right).
\end{equation}

Hence if we take
\[
	n = \frac{2k}{\eps}, R = \frac{\log^2 (\frac{2k}{\eps} + 1)}{ \eps ^2},
\]

we can get $|\Ent{p} - \Expc{\widehat{H}} | \le \eps $ with probability at least $3/4$. The total number of samples used is $nR = O\left (\frac{k \log^2 k}{\eps^3} \right )$Our result is summerized in the following theorem:

 \begin{theorem}\label{thmnaive}
 Algorithm~\ref{alg1} uses $O\left(1\right)$ words of memory and its sample complexity is 
 \begin{equation}
 \SamC{k}{\eps}{\frac{1}{4}} = O\left(\frac{k \log^2 k}{\eps^3}\right).
 \end{equation}
 \end{theorem}

The proof directly follows from the analysis. From Lemma~\ref{lem:mdlbias}, $n$, number of samples controls the bias term and $R$ controls the concentration term of the error. And the complexity bound $nR$ comes from treating each individual symbol equally and consider the worst case over all symbols. However, if we use different $n$'s and $R$'s for different symbols. For $x$'s with larger probability, we can make $n$ smaller since its easier to control the bias and for $x$'s with smaller probability, we can make $R$ smaller since its easier to control the variance because $\widehat{H}$'s will be in a smaller range with high probability. We will make this intuition concrete in the next section and see how we can use this to reduce sample complexity.
}

\end{comment}

%The entropy of a random variable $X \sim p$ is the expectation of $\log \left(1/p\left(X\right) \right)$ taken with respect to $p\left(x\right)$. Algorithm~\ref{alg1} estimates this expectation by computing the average of $\log \left(1/p\left(X\right) \right)$ over $\vSmp = \Omega\left(\frac{\log^2\left(k\right)}{\eps^2}\right)$ samples. For each of the $\vSmp$ samples, $\bSmp = \Omega\left(\frac{k}{\eps}\right)$ samples are used to compute an empirical estimate of $\log \left(1/p\left(X\right) \right)$. \par
%We now present an alternative view of the entropy estimate $\widehat{H}$ of Algorithm~\ref{alg1} in terms of its bias $ \left \lvert \Ent{p} -  \Expc{ \widehat{H}} \right \rvert$  and concentration $ \left \lvert \widehat{H} -  \Expc{ \widehat{H}} \right \rvert$. Since $\widehat{H}$ is an average over $\vSmp$ samples, $\vSmp$ can be thought of as a parameter that controls the concentration of $\widehat{H}$. By Hoeffding's inequality, $\vSmp$ depends on the range of the estimate of  $\log \left(1/p\left(X\right) \right)$ which is $\sim \log n$.  Since Algorithm~\ref{alg1} uses $\bSmp$ samples to estimate $\log \left(1/p\left(X\right) \right)$, $\bSmp$ can be thought of as a parameter that controls the bias of $\widehat{H}$.
%
%%\begin{algorithm}
%%\caption{Entropy estimation : Model Algorithm} \label{alg1_old}
%%\begin{algorithmic}[1]
%%\State $\widehat{H}= 0$ 
%%\For{$t=1 \cdots \vSmp = \frac{\log^2 \left(\frac{2k}{\eps}+1\right)}{\eps^2} $}
%%	\State Sample $x_t \sim p$ 
%%	\State $N_{x_t} = 0$
%%	\For{$i=1 \cdots \bSmp = \frac{2k}{\eps}$}
%%		\State Sample $x_i \sim p$ 
%%		\If{$x_i = x_t$}
%%			\State $N_{x_t} = N_{x_t} + 1$
%%		\EndIf
%%	\EndFor
%%	\State $\widehat{H} = \widehat{H} + \log\left(\dfrac{\bSmp}{N_{x_t} + 1}	\right)$		 \label{entstepalg1}
%%\EndFor
%%\State $\widehat{H} = \dfrac{\widehat{H}}{\vSmp}$
%%\end{algorithmic}
%%\end{algorithm}
% 
%%Thm Statement 
% \begin{theorem}\label{thmnaive}
% Algorithm~\ref{alg1} uses $O\left(1\right)$ words of memory and its sample complexity is 
% \begin{equation}
% \SamC{k}{\eps}{\frac{1}{4}} = O\left(\frac{k \log^2 k}{\eps^3}\right).
% \end{equation}
% \end{theorem}
% 
% %Proof 
% \begin{proof}
% Since Algorithm~\ref{alg1} does not store more than two samples at an instance it uses $O\left(1\right)$ words. Since $\widehat{H}$ is an average over $\vSmp$ samples and for each such sample, $\bSmp$ more samples are used to estimate $\log \left(1/p\left(X\right) \right)$, the total sample complexity of $\widehat{H}$ is $\bSmp \vSmp = O\left(\dfrac{k\log^2\left(k\right)}{\eps^3}\right)$. \par 
% Finally, to prove that with probability atleast $3/4$, $\lvert \Ent{p} - \widehat{H} \rvert \leq \eps$, we  bound the bias and the concentration of $\widehat{H}$ in the following lemmas whose proofs are deferred to Section~\ref{sec:mdlpfs}.
% 
% \begin{lemma}(\textbf{Bias Bound})\label{lem:mdlbias}
% For the entropy estimate of Algorithm~\ref{alg1},
% \begin{equation}
% \left \lvert \Ent{p} - \Expc{\widehat{H}} \right \rvert \leq \frac{k}{\bSmp} \leq \frac{\eps}{2}.
% \end{equation}
% \end{lemma}
%  
% \begin{lemma}(\textbf{Concentration Bound})\label{lem:mdlconc}
% For the entropy estimate of Algorithm~\ref{alg1},
% \begin{equation}
% \Pr \left( \left \lvert \widehat{H} - \Expc{\widehat{H}} \right \rvert \geq  \frac{\eps}{2} \right) \leq \exp \left(- \frac{R\eps^2}{2\log^2 \left(n+1\right)} \right) \leq \frac{1}{4}.
% \end{equation}
%  \end{lemma}
%  
%%Therefore, from equation \eqref{bias} and equation \eqref{cnvrge},
%%\begin{align}
%%n &= O\left(\frac{k}{\eps}\right) \\
%%R &= O\left(\frac{\log^2 \left(n+1\right)}{\eps^2} \right)
%%\end{align}
%
% \end{proof}
%
%%We now present some intuition that we will use to improve the sample complexity of the model algorithm. Let $\ell$ be such that $\frac{1}{k} \leq \ell < \frac{1}{2}$. If we knew beforehand that for some symbols $x$, $p\left(x\right) \geq \ell $, it would be easier to estimate $\log\left(1/p(X)\right)$ since the probability of these symbols is high. In other words, we could use a smaller value of $\bSmp$ for such symbols since their contribution to the bias would be small. On the other hand, for symbols such that $p\left(x\right) \leq \ell $, we could use a smaller value of $\vSmp$ since the interval is smaller.

==> two-intervals__Sourbh_Bhadane_s_conflicted_copy_2019-11-12_.tex <==
\new{The algorithm in the previous section treats each symbol equally and uses the same $N$ and $R$.} 
%To reduce the sample complexity, we make the following thought experiment. Suppose we are guaranteed that all probability values $p(x)$ are at most $(\log k)^\beta/k$ for some positive integer $\beta$. Then, we know that the contribution that each symbol makes to the entropy term is at most $\log k -\beta \log \log k$. We can therefore hope that the number of iterations $R$ needed for these intervals can be made smaller. If there are probability values larger than  $(\log k)^\beta/k$ we should be able to estimate their values with smaller $N$ than needed earlier. 
To reduce the sample complexity, our high level approach is the following:
\begin{itemize}
\item Let $T\in\NN$, and $0=\prt_0<\prt_1<\ldots<\prt_T=1$. We design a partition $\mathcal{I} := \{I_1, I_2, ..., I_T\}$ of $\left[0,1 \right]$ into $T$ intervals with $I_j = [a_{T-j}, a_{T-j+1})$. 
\item
We will express the entropy as an expectation of entropy-like terms over these intervals (Lemma~\ref{lem:decom}), and will estimate the contribution from each interval.
\item Consider the $j$th interval, $I_j = [a_{T-j}, a_{T-j+1})$. For $p(x)\in I_j$, 
%note that $p(x)\in (\log (1/a_{T-j+1}), \log (1/a_{T-j})]$. 
the number of samples needed to estimate $p(x)$ grows roughly as $1/a_{T-j}$. Therefore, intervals close to zero need more samples, and intervals far from zero require fewer samples.  
\item
Note that for $p(x)\in I_j, \log (1/p(x)) \in (\log (1/a_{T-j+1}), \log (1/a_{T-j})]$. We choose the intervals such that this width decreases for intervals close to zero. In doing so, we will ensure that while more samples are needed to estimate the probability values in these intervals, we need fewer iterations (small $R$) to estimate the contribution of these intervals to entropy. 
\end{itemize}

\begin{figure}[H]
\begin{center}
\begin{tikzpicture}[xscale=12]
\draw[-][ultra thick] (0,0) -- (1,0);
\draw [ultra thick] (0,-.1) node[below]{$a_0 = 0$} -- (0,0.1);
\draw [ultra thick] (0.166,-.1) node[below]{$a_1$} -- (0.166,0.1);
\node[below] at (0.333,-.1) {$\cdots$};
%\draw [ultra thick] (0.40,-.1) node[below]{$a_{T-j}$} -- (0.40,0.1);
\draw [ultra thick] (0.50,-.1) node[below]{$a_{T-j}$} -- (0.50,0.1);
\draw [ultra thick] (0.666,-.1) node[below]{$a_{T-j+1}$} -- (0.666,0.1);
,\draw [ultra thick] (0.833,-.1) node[below]{$a_{T-1}$} -- (0.833,0.1);
\draw [ultra thick] (1,-.1) node[below]{$a_T = 1$} -- (1,0.1);
\node[above] at (0.08,0.2) {$I_T$};
\node[above] at (0.57,0.2) {$I_j$};
\node[above] at (0.90,0.2) {$I_1$};
\end{tikzpicture}
\caption{Partition of $\left[0,1\right]$ into $T$ intervals}
\end{center}
\end{figure}
%To reduce the sample complexity, we express $H(p)$ as an expectation of various conditional expectations depending on the symbol probability values. For larger probability values we use smaller $N$ and for small probabilities we use smaller $R$. We then estimate the terms separately to obtain the final estimate.
\noindent In Lemma~\ref{lem:decom} we express entropy as a summation over the contributions from the various intervals. 

\noindent\textbf{Entropy as a Weighted Sum of Conditional Expectations.}\label{subsec:condexp}
Ideally, our approach (similar to the previous section) would be the following. Obtain a symbol in the data stream, find which interval it lies in, and estimate the entropy contribution from each interval separately. However, we may not be able to estimate the exact interval that a symbol is in. To take care of this, consider a randomized algorithm $\mathcal{A}:[k]\to\{I_1,\ldots, I_T\}$ that takes as input $x\in[k]$, and outputs an interval in $\cI$ (which corresponds to our guess for the interval in which $p(x)$ lies in). For a symbol $x$, let $p_{\cA}\left(I_j \middle| x \right) := \probof{\cA(x) = I_j}$ be the distribution of the output of $\mathcal{A}$ for a symbol $x$. For a distribution $\p\in\Delta_k$, let
%\vspace{-5pt}
\begin{align} \label{eq:conddist}
p_\cA\Paren{I_j} := \sum_{x\in [k]}\p(x)\cdot p_{\cA}\left(I_j \middle| x \right), && p_\cA\left(x \middle| I_j \right) := \frac{\p(x)\cdot p_{\cA}\left(I_j \middle| x \right)}{p_\cA\left(I_j \right) }.
\end{align}
Then $p_\cA\Paren{I_j}$ is the probability that $\cA(X)=I_j$, when $X\sim\p$. $p_\cA\left(x \middle| I_j \right)$ is the distribution over $[k]$ conditioned on $\cA(X)= I_j$. . 

For any randomized function $\mathcal{A}:[k]\to\{I_1,\ldots, I_T\}$ we can characterize the entropy as follows. 
\begin{lemma} \label{lem:decom}
	%\begin{align}\vspace{-2ex}
	Let $ H_j := \EE _{X \sim p_\cA \left(x \middle| I_j \right)}\left[ -\log{p\left(X\right)}  \right]$ then, $\Ent{p} = \sum_{j=1}^{T} p_\cA\left(I_j \right)  H_j.$ \label{entintexp}
	%	\end{align}
\end{lemma}
\begin{proof}
\begin{align}
\Ent{\p}  = \sum_x \p(x) \Paren{\sum_j p_{\cA}\left(I_j \middle| x \right)}\log \frac1{\p(x)} &= \sum_x  \sum_j \Paren{p_\cA\left(I_j \right) p_\cA\left(x \middle| I_j \right) \log \frac1{\p(x)}}\label{eqn:mid-step-ent-decomp}\\
&= \sum_j p_\cA\Paren{I_j} \Paren{ \EE _{X \sim p_\cA \left(x \middle| I_j \right)}\left[ -\log{p\left(X\right)}  \right]}.\nonumber
\end{align}	
where~\eqref{eqn:mid-step-ent-decomp} follows from~\eqref{eq:conddist}. 
\end{proof}
Suppose $\cA$ is such that it outputs the exact interval in which $p(x)$ is in, then $p_\cA\Paren{I_j}=p(I_j)$, the total probability of interval $I_j$, and $p_\cA(x|I_j)$ is the conditional distribution of all symbols in $I_j$. In this case, the lemma above reduces to the grouping property of entropy~\cite{CoverT06}. In our streaming setting, the algorithm $\cA$ will take as input an element $x$ of the data stream, and then based on the number of occurrences of $x$ over a window of certain size in the subsequent stream outputs an interval in $\cI$. 
%Suppose $X\sim \p$, then the event $\{\cA(X)\in I_j\}$ induces a conditional distribution over $[k]$,
%%\vspace{-5pt}
%\begin{align}
%p_\cA\left(x \middle| I_j \right) := \frac{\p(x)\cdot p_{\cA}\left(I_j \middle| x \right)}{p_\cA\left(I_j \right) }.\label{eqn:cond-dist}
%\end{align}
%\vspace{-10pt}
%\noindent\textbf{Entropy as a Conditional Expectation.}\label{subsec:condexp}
%Let $T\in\NN$ (decided later), and $0=\prt_0<\prt_1<\ldots<\prt_T=1$. This partitions $\left[0,1 \right]$ into $T$ intervals $\mathcal{I} = \{I_1, I_2, ..., I_T\}$, where $I_j = [a_{T-j}, a_{T-j+1})$. 
%
%Consider a randomized algorithm $\mathcal{A}:[k]\to\{I_1,\ldots, I_T\}$ that takes as input $x\in[k]$, and outputs an interval in $\cI$. For a distribution $\p\in\Delta_k$, let
%%\vspace{-5pt}
%\begin{equation} \label{eq:conddist}
%	p_\cA\Paren{I_j} := \sum_{x\in [k]}\p(x)\cdot \probof{\cA(x) = I_j},
%\end{equation}
%be the probability that $\cA(X)=I_j$, when $X\sim\p$.  We will denote $ \probof{\cA(x) = I_j}$ as $p_{\cA}\left(I_j \middle| x \right)$.
%Suppose $X\sim \p$, then the event $\{\cA(X)\in I_j\}$ induces a conditional distribution over $[k]$,
%%\vspace{-5pt}
%	\begin{align}
%		p_\cA\left(x \middle| I_j \right) := \frac{\p(x)\cdot p_{\cA}\left(I_j \middle| x \right)}{p_\cA\left(I_j \right) }.\label{eqn:cond-dist}
%	\end{align}
%%\vspace{-10pt} we have the following lemma:

%\begin{align}
%\Ent{\p}  = \sum_x \p(x) \Paren{\sum_j p_{\cA}\left(I_j \middle| x \right)}\log \frac1{\p(x)} &= \sum_x  \sum_j \Paren{p_\cA\left(I_j \right) p_\cA\left(x \middle| I_j \right) \log \frac1{\p(x)}}\label{eqn:mid-step-ent-decomp}\\
%&= \sum_j p_\cA\Paren{I_j} \Paren{ \EE _{X \sim p_\cA \left(x \middle| I_j \right)}\left[ -\log{p\left(X\right)}  \right]},\nonumber
%\end{align}	
%where~\eqref{eqn:mid-step-ent-decomp} follows from~\eqref{eq:conddist}. 
%\vspace{-10pt}
%\begin{align}
%\Ent{\p} = \sum_x \p(x)\log \frac1{\p(x)}&= \sum_x \p(x) \Paren{\sum_j p_{\cA}\left(I_j \middle| x \right)}\log \frac1{\p(x)}\nonumber\\
%& = \sum_x  \sum_j \Paren{ \p(x)p_{\cA}\left(I_j \middle| x \right) \log \frac1{\p(x)}}\nonumber\\
%& = \sum_x  \sum_j \Paren{p_\cA\left(I_j \right) p_\cA\left(x \middle| I_j \right) \log \frac1{\p(x)}}\label{eqn:mid-step-ent-decomp}\\
%& = \sum_j p_\cA\Paren{I_j}  \Paren{\sum_x p_\cA\left(x \middle| I_j \right) \log \frac1{\p(x)}}\nonumber\\
%& = \sum_j p_\cA\Paren{I_j} \Paren{ \EE _{X \sim p_\cA \left(x \middle| I_j \right)}\left[  \log\frac{1}{p\left(X\right)}  \right]},\nonumber
%\end{align}	
%Now, we can rewrite the entropy in terms of these distributions as follows.
%\begin{align}
%\Ent{\p} = \EE_{X\sim p} \left[  \log \left(\frac{1}{\p(X)}\right)\right] &= \EE_{I_j \sim p_\cA\Paren{I}} \left[\EE_{X \sim p_\cA \left(x \middle| I_j \right)} \left[  \log \left(\frac{1}{\p(X)}\right)\right] \right]\nonumber \\
%&= \sum_j p_\cA\Paren{I_j} \Paren{ \EE _{X \sim p_\cA \left(x \middle| I_j \right)}\left[  \log\frac{1}{p\left(X\right)}  \right]}.\nonumber
%\end{align}	
% Defining
%% \vspace{-5pt}
%\begin{align}
% H_j := \EE _{X \sim p_\cA \left(x \middle| I_j \right)}\left[ -\log{p\left(X\right)}  \right]\label{eqn:hj-def},
% \vspace{-5pt}
%\end{align}
%  \vspace{-5pt}

%Our approach would be to estimate each term in the summation above, and output their summation. In the previous section, we considered $T=1$, namely all the symbols are treated identically. By choosing the intervals appropriately, we will show that there is an algorithm that uses $O(k (\log^{(T)} (k/\eps))^2/\eps^3)$ samples and a constant words of space, and estimates $H(\p)$ to $\pm\eps$. For $T=1$, $\log^{(T)} k = \log k$, and for $T\ge 1$, $\log^{(T)} k = \max\{\log (\log^{(T-1)} k), 1\}$. 

%By choose the intervals and algorithm $\cA$ appropriately, and estimating each term in the summation above, we will show that there is an algorithm that satisfies the constraints in Theorem~\ref{thm:main_perf}.

We will choose the intervals and algorithm $\cA$ appropriately. By estimating each term in the summation above, we will design an algorithm with $T$ intervals that uses $O\Paren{\frac{k (\log^{(T)} k + \log(1/\eps))^2}{\eps^3}}$ 
 samples and a constant words of space, and estimates $H(\p)$ to $\pm\eps$ with probability at least $2/3$. Here $\log ^{(T)}$ denotes the iterated logarithms, and therefore shows the improvement in logarithmic terms as $T$ grows. 

In Section~\ref{sec:two_interval}, we provide the details with $T=2$. %, and obtain an algorithm with sample complexity $O(\frac{k (\log (\log (k)/\eps))^2}{\eps^3})$, which improves the sample requirements of Theorem~\ref{thm:one-interval} from a single $\log$, to $\log \log$. 
This section will flesh out the key arguments, and show how to reduce the $\log k$ term in the previous section to $\log \log k$. Finally in Section~\ref{sec:general_interval}, we extend this to $T = \log^* k$ where $\log^* k= \min_i \{\log^{(i)} k \le 1\} $ intervals to further reduce the sample complexity to $O({k (\log (1/\eps))^2}/{\eps^3})$.

\subsection{Two Intervals Algorithm ($T=2$)} \label{sec:two_interval}

We propose Algorithm~\ref{alg:twoint} with the following guarantee. 
%\vspace{-5pt}
\begin{theorem} \label{thm:perf_two}
	Algorithm~\ref{alg:twoint} uses 
	%\begin{align}
	%n_2 &= C_1 \cdot \frac{k}{\eps}, \hspace{5mm} n = n_1 = C_1 \cdot\frac{k}{\eps \left( \log k \right)^{\gamma} }. \label{eqn:defn}\\
	%R_2 &= C_2 \cdot \frac{\left(\log \log k\right)^2}{\epsilon^2}, \hspace{5mm} R = R_1 = C_2 \frac{\log^2 k}{\eps^2}. \label{eqn:defr}
	%\end{align}
	%with proability at least 2/3, we have:
	%\[	|\Ent{p} -  \estII| \le \eps \]
$
		O(NR + N_1R_1 + N_2R_2) = O\left( \frac{k (\log \left(\log (k)/\eps\right))^2}{\eps^3}\right)
$
	samples, $20$ words and outputs an $\pm\eps$ estimate of $H(p)$ with probability at least $2/3$.
\end{theorem}
%\vspace{-10pt}

\subsubsection{Description of the Algorithm}
Let $T=2$, and $\beta>16$ be a constant. Consider the following partition of $\left[0 ,1\right]$:
%\vspace{-10pt}
\begin{equation}
I_2 = \left[0,\ell \right), I_1 = \left[\ell,1\right] \hspace{5mm} \text{where} \hspace{5mm} \ell = {\left(\log k \right)^{\beta}}/{k}.\label{eqn:two-ints}
\end{equation}

\begin{figure}[H]
\begin{center}
\begin{tikzpicture}[xscale=12]
\draw[-][ultra thick] (0,0) -- (1,0);
\draw [ultra thick] (0,-.1) node[below]{$0$} -- (0,0.1);
\draw [ultra thick] (0.35,-.1) node[below]{$\ell = \frac{(\log k)^{\beta}}{k}$} -- (0.35,0.1);
\draw [ultra thick] (1,-.1) node[below]{$1$} -- (1,0.1);
\node[above] at (0.2,0.2) {$I_2$};
\node[above] at (0.65,0.2) {$I_1$};
\end{tikzpicture}
\caption{Partition of $\left[0,1\right]$ into two intervals}
\end{center}
\end{figure}
We now specify the algorithm $\cA:[k]\to\{I_1, I_2\}$ we used in Lemma~\ref{lem:decom}. $\cA$ is denoted by $\textsc{EstInt}$ (Algorithm~\ref{alg:intvlesti}). %t essentially tries to \emph{guess the interval} in which the probability of $x$ lies. 
For $x\in[k]$, it takes $\bSmp$ samples from $\p$, and if the fraction of occurrences of $x$ is more than $\ell$ it outputs $I_1$, else it outputs $I_2$. This is an algorithm that tries to guess the true interval containing $p(x)$ from the samples.
%\begin{minipage}[t]{0.45\textwidth}
%\null
%\begin{algorithm}[H]
%	\caption{$\cA$ : $\textsc{EstInt} \left(\bSmp, x\right)$} \label{alg:intvlesti}
%	\begin{algorithmic}[1]
%		\Require $\bSmp$, $x\in [k]$
%		\State Obtain $\bSmp$ samples from $p$ 
%		\State { \textbf{if} $x$ appears $\geq \bSmp\ell$ times output $I_1$}
%		\State { \textbf{else} output $I_2$}
%	\end{algorithmic}
%\end{algorithm} 
%\end{minipage}
%%\hfill
%\begin{minipage}[t]{0.45\textwidth}
%\null
%\begin{algorithm}[H]
%	\caption{ $\textsc{EstProbInt}\left(\bSmp, \vSmp\right)$} \label{alg:est_p1}
%	\begin{algorithmic}[1]
%		\Require $\bSmp, \vSmp$
%		\State $\widehat{p}_\cA\left(I_1 \right) = 0$
%		\For{$t = 1 \text{ to } \vSmp$}
%		\State Sample $x \sim \p$.
%		\State {\textbf{if} $\textsc{EstInt}\left(\bSmp, x\right) = I_1$}
%		\State {\textbf{then} $\widehat{p}_\cA\left(I_1 \right)= \widehat{p}_\cA\left(I_1 \right)+ \frac{1}{\vSmp}$}
%		\EndFor
%	\end{algorithmic}
%\end{algorithm} 
%\end{minipage}
\begin{table}[ht]
	\vspace{-20pt}
	\begin{tabular}{cc}
		\begin{minipage}[t]{0.4\textwidth}
		\begin{algorithm}[H]
		\caption{$\cA$ : $\textsc{EstInt} \left(\bSmp, x\right)$} \label{alg:intvlesti}
		\begin{algorithmic}[1]
%		\Require $\bSmp$, $x\in [k]$
		\State Obtain $\bSmp$ samples from $p$ 
		\State { \textbf{if} $x$ appears $\geq \bSmp\ell$ times, output $I_1$}
		\State { \textbf{else} output $I_2$}
		\end{algorithmic}
		\end{algorithm} 
		\end{minipage}
%\hfill
		&
		\begin{minipage}[t]{0.5\textwidth}
%\null
		\begin{algorithm}[H]
		\caption{ $\textsc{EstProbInt}\left(\bSmp, \vSmp\right)$} \label{alg:est_p1}
		\begin{algorithmic}[1]
%		\Require $\bSmp, \vSmp$
		\State $\widehat{p}_\cA\left(I_1 \right) = 0$
		\For{$t = 1 \text{ to } \vSmp$}
		\State Sample $x \sim \p$.
		\If {$\textsc{EstInt}\left(\bSmp, x\right) = I_1$}
		 \State $\widehat{p}_\cA\left(I_1 \right)= \widehat{p}_\cA\left(I_1 \right) + {1}/{\vSmp}$
		 \EndIf
		\EndFor
		\end{algorithmic}
		\end{algorithm} 
		\end{minipage}
\end{tabular}
\end{table}
%We can see if we choose $n$ large enough, then with a high probabiltiy, $EstInt(n,x) = I_1$ if $\p(x) > 2n\ell $ and $EstInt(n,x) = I_2$ if $\p(x) < n\ell/2 $. This seperation will help us reduce the number of samples needed to estimate $H_1$ and $H_2$. Next we will see how to estimate $p_\cA\left(I_1 \right), p_\cA\left(I_2 \right)$  and $H_1, H_2$.

By Lemma~\ref{lem:decom}, $
	\Ent{p} =  p_\cA\left(I_1 \right)  H_1 +p_\cA\left(I_2 \right)  H_2.$
We estimate the terms in this expression as follows. 
%\medskip

\medskip
\noindent\textbf{Estimating $p_\cA(I_j)$'s.} We run $\textsc{EstInt}$ multiple times on samples generated from $\p$, and output the fraction of times the output is $I_j$ as an estimate of $\p_\cA(I_j)$. We only estimate $p_\cA(I_1)$, since $p_\cA(I_1)+p_\cA(I_2)=1$. The complete procedure %for estimating the probabilities are given below, and it takes two parameters $\bSmp$, and $R$. This 
is specified in Algorithm~\ref{alg:est_p1}.
%\begin{algorithm}[ht]
%	\caption{Estimating $p_\cA\left(I_1 \right), p_\cA\left(I_2 \right)$ : $\textsc{EstProbInt}\left(\bSmp, \vSmp\right)$} \label{alg:est_p1}
%	\begin{algorithmic}[1]
%		\Require $\bSmp, \vSmp$
%		\State $\widehat{p}_\cA\left(I_1 \right) = 0$
%		\For{$t = 1 \text{ to } \vSmp$}
%		\State Sample $x \sim \p$.
%		\State {\textbf{if} $\textsc{EstInt}\left(\bSmp, x\right) = I_1$ \textbf{then} $\widehat{p}_\cA\left(I_1 \right)= \widehat{p}_\cA\left(I_1 \right)+ \frac{1}{\vSmp}$}
%		\EndFor
%	\end{algorithmic}
%\end{algorithm} 

\medskip
\noindent\textbf{Estimating $H_j$'s.} Recall that $H_j$'s are the expectations of $-\log \left({p(x)}\right)$ under different distributions given in~\eqref{eq:conddist}. %Even though we do not know these distributions, we can generate samples from them using $\cA$, and then estimate the probability of the sample thus generated by taking more samples from the underlying $\p$.  
Since the expectations are with respect to the conditional distributions, we first sample a symbol from $p$ and then conditioned on the event that $\textsc{EstInt}$ outputs $I_j$, we use an algorithm similar to Algorithm~\ref{alg1} to estimate $\log (1/\p(x))$. The complete procedure is given in Algorithm~\ref{alg:hi_est2}. Notice that when computing $\widehat{H}_2$ in Step~\ref{step:clip}, we clip the $\widehat{H}_2$'s to $\log \frac{1}{4\ell}$ if $N_{x,2} > 4\ell \bSmp_2 -1$. This is done to restrict each $\widehat{H}_2$ to be in the range of $[\log \frac{1}{4\ell}, \log \bSmp_2]$, which helps in obtaining the concentration bounds by bounding the width of the interval for applying Hoeffding's inequality. 
\begin{algorithm}[ht]
	\caption{Estimating $H_1$ and $H_2$ : $\textsc{CondExp}\left(\bSmp_1, \bSmp_2, \vSmp_1, \vSmp_2\right)$} \label{alg:esthi}
	\label{alg:hi_est2}
	\begin{algorithmic}[1]
		\For{$i=1,2$, set $\widehat{H}_i = 0, S_i = 0$, }
		%\State 
		\For{$t=1 \text{ to } R_i$}
		\State Sample $x \sim \p$
		\If{$\textsc{EstInt}\left(\bSmp, x\right)=I_i$} \label{lst:line:esthicond}
		\State $S_i = S_i + 1$
		\State Let $N_{x,i} \leftarrow$ \# occurrences of $x$ in the next $\bSmp_i$ samples  \label{computehl2}
		\State $\widehat{H}_i = \widehat{H}_i + \log \left(\bSmp_i/(N_{x,i} + 1) \right)$ if $i = 1$
		\State $\widehat{H}_i = \widehat{H}_i + \max \left\{\log \left(\bSmp_i/(N_{x,i} + 1)\right), \log \Paren{1/4\ell} \right\} $ if $i = 2$ \label{step:clip}
		\EndIf
		\EndFor
		\State $\bar{H}_i =\widehat{H}_i/S_i$
		\EndFor
	\end{algorithmic}
\end{algorithm} 
%\begin{table}[ht]
%	\begin{tabular}{cc}
%		\begin{minipage}[t]{0.45\textwidth}
%\begin{algorithm}[H]
%	\caption{$\textsc{CondExp}\left(\bSmp_1, \bSmp_2, \vSmp_1, \vSmp_2\right)$} \label{alg:esthi}
%	\begin{algorithmic}[1]
%		\For{$i=1,2$}
%		\State $\widehat{H}_i = 0, S_i = 0$
%		\For{$t=1 \text{ to } R_i$}
%		\State Sample $x \sim \p$
%		\If{$\textsc{EstInt}\left(\bSmp, x\right)=I_i$} \label{lst:line:esthicond}
%		\State $S_i +=  1$
%		\State Let $N_{x,i} \leftarrow$ \# occurences of $x$ in the next $\bSmp_i$ samples  \label{computehl2}
%		\State $\widehat{H}_i += \log \left(\frac{\bSmp_i}{N_{x,i} + 1} \right)$ if $i = 1$
%		\State $\widehat{H}_i += \max \left\{\log \left(\frac{\bSmp_i}{N_{x,i} + 1}\right), \log \Paren{\frac{1}{4\ell}} \right\} $ if $i = 2$ \label{step:clip}
%		\EndIf
%		\EndFor
%		\State $\bar{H}_i = \frac{\widehat{H}_i}{S_i}$
%		\EndFor
%	\end{algorithmic}
%\end{algorithm} 
%\end{minipage}
%&
%\begin{minipage}[t]{0.45\textwidth}
%\begin{algorithm}[H]
%	\caption{Two Intervals Algorithm} \label{alg:twoint}
%	\begin{algorithmic}[1]
%	\Require $\eps>0, \gamma=\beta/2$, $X_1, X_2, \ldots\sim p$
%		\State Set 
%		%\vspace{-10pt}
%		\[
%		\bSmp = \bSmp_1 = C_1 \cdot\frac{k}{\eps \left( \log k \right)^{\gamma} }, \vSmp = \vSmp_1 = C_2 \frac{\log(k/\eps)^2 }{\eps^2}
%		\]
%		%\vspace{-10pt}
%		\[ 
%		\bSmp_2 = C_1 \cdot \frac{k}{\eps}, \vSmp_2 = C_2 \cdot \frac{\left(\log ((\log k)/\eps)\right)^2}{\eps^2}
%		\] \label{step:params}
%		%\vspace{-15pt}
%		\State $\widehat{p}_\cA\left(I_1 \right)= \textsc{EstProbInt}\left(\bSmp,\vSmp \right)$
%		\State $\bar{H}_1, \bar{H}_2 = \textsc{CondExp}\left(\bSmp_1, \bSmp_2, \vSmp_1, \vSmp_2 \right) $
%		\State $\estII = \widehat{p}_\cA\left(I_1 \right)\bar{H}_1 + (1-\widehat{p}_\cA\left(I_1 \right))\bar{H}_2  $
%	\end{algorithmic}
%\end{algorithm}
%\end{minipage}
%\end{tabular}
%\end{table}


%Our estimate for $\Ent{p}$ is simply:
%\begin{equation} \label{eqn:estimation_two}
%\estII= \widehat{p}_\cA\left(I_1 \right) \bar{H}_1 + (1 - \widehat{p}_\cA\left(I_1 \right) )\bar{H}_2
%\end{equation}

%\noindent\textbf{Complete algorithm for $T=2$.}
%%We specify the complete procedure for $T=2$ in Algorithm~\ref{alg:twoint}. The algorithm specifies the choice of parameters used to compute the estimated probabilities and $H_j$'s, which are then used to estimate $H(\p)$.  Note that $\bSmp_2 > \bSmp_1$ and $\vSmp_2 < \vSmp_1$.
%%We note that for $I_2$, we use a relatively larger $\bSmp_2$ but a smaller $\vSmp_2$ while for $I_1$ we are using a larger $\vSmp_1$ and smaller $\bSmp_1$.  
%Algorithm~\ref{alg:twoint} contains the complete procedure with the choice of parameters used to compute $\widehat{p}_\cA\left(I_1 \right)$ and $\bar{H}_j$'s, which are then used to estimate $H(\p)$.  Note that $\bSmp_2 > \bSmp_1$ and $\vSmp_2 < \vSmp_1$.

\begin{algorithm}[t]
	\caption{Entropy Estimation with constant space: Two Intervals Algorithm} \label{alg:twoint}
	\begin{algorithmic}[1]
	\Require Accuracy parameter $\eps>0, \gamma=\beta/2$, a data stream $X_1, X_2, \ldots\sim p$
		\State Set 
		\vspace{-10pt}
		\[
		\bSmp = \bSmp_1 = \frac{C_1 k}{\eps \left( \log k \right)^{\gamma} },\ \vSmp = \vSmp_1 = C_2 \frac{\log(k/\eps)^2 }{\eps^2},\ 
%		\]
%		%\vspace{-10pt}
%		\[ 
		\bSmp_2 = C_1 \cdot \frac{k}{\eps},\  \vSmp_2 = C_2 \cdot \frac{\left(\log ((\log k)/\eps)\right)^2}{\eps^2}
		\] \label{step:params}
		%\vspace{-15pt}
		\State $\widehat{p}_\cA\left(I_1 \right)= \textsc{EstProbInt}\left(\bSmp,\vSmp \right)$
		\State $\bar{H}_1, \bar{H}_2 = \textsc{CondExp}\left(\bSmp_1, \bSmp_2, \vSmp_1, \vSmp_2 \right) $ \label{step:est_ent}
		\State $\estII = \widehat{p}_\cA\left(I_1 \right)\bar{H}_1 + (1-\widehat{p}_\cA\left(I_1 \right))\bar{H}_2  $
	\end{algorithmic}
\end{algorithm}


%\medskip
%\noindent\textbf{Memory Requirements for Algorithm~\ref{alg:intvlesti}.}
%One word is required to store the input symbol $x$ and one word each to store the counter and one symbol from the stream of $\bSmp$ samples. Another word is required to count  the number of times $x$ appears in the $\bSmp$ samples. 

\subsubsection{Performance Guarantees}
%\textbf{Memory Requirements.} We reserve 5 words to store parameters $\vSmp_1, \vSmp_2, \bSmp_1, \bSmp_2$ and $\ell$.
% \textsc{EstInt} uses one word to keep track of the number of occurrences of $x$. For \textsc{EstProbInt}, we use one word to store $x$ and one word to keep track of the final sum $\widehat{p}_{\cA}\left(I_1\right)$. We execute \textsc{CondExp} for each interval separately and  use one word each to store $x$ and keep track of $S_i$ and $\widehat{H_i}$. We use two words to store the outputs $\bar{H_1}$ and $\bar{H_2}$ and store the final output $\widehat{H}_{II}$ in one of those. Hence, at most 20 words of memory are sufficient.
\textbf{Memory Requirements.} Since $\vSmp_1, \vSmp_2, \bSmp_1, \bSmp_2$ and $\ell$ are program constants, we compute them on execution by storing $k,\eps, C_1,C_2, \gamma$ using five words in total.
\begin{itemize}
\item \textsc{EstInt} uses two words for the counter and two words to keep track of number of appearances of $x$. These four words are reused on each invocation of \textsc{EstInt}. 
\item \textsc{EstProbInt} uses two words to store the counter and one word to store the final output.
\item \textsc{CondExp} is executed for each interval separately which allows reusing the memory required for one iteration. Storing the counter, $x$, $S_i$ requires two, one and two words respectively. The final answer requires two words to store. 
\end{itemize}
Hence, at most 20 words of memory are sufficient. 

%For all parameters on Line~\ref{step:params}, we reserve two words and compute them on the fly. It is sufficient to use two words to store one of $\widehat{p}_{\cA}\left(I_1\right)$ and $\widehat{p}_{\cA}\left(I_2\right)$, and one of $\widehat{H}_1$ and $\widehat{H}_2$ since both $\textsc{EstProbInt}$ and $\textsc{CondExp}$ can be executed for each interval together. We use one word to store the final estimate $\estII$. \textsc{EstInt} uses one word each to store $x$, a symbol of the stream of $\bSmp$ samples, the interval, and to count occurrences of $x$. \textsc{CondExp} requires four more words to store $i,S_i,N_i,N_{x,i}$. None of the algorithms require more than three counters at once for which we use four words in total. Hence, at most 20 words of memory are required.

%\medskip
%\noindent \textbf{Memory Requirements for Algorithm~\ref{alg:twoint}.} 
%For all parameters on Line~\ref{step:params}, we reserve two words and compute them on the fly. It is sufficient to use two words to store one of $\widehat{p}_{\cA}\left(I_1\right)$ and $\widehat{p}_{\cA}\left(I_2\right)$, and one of $\widehat{H}_1$ and $\widehat{H}_2$ since both $\textsc{EstProbInt}$ and $\textsc{CondExp}$ can be executed for each interval together. We use one word to store the final estimate $\estII$. \textsc{EstInt} uses one word each to store $x$, a symbol of the stream of $\bSmp$ samples, the interval, and to count occurrences of $x$. \textsc{CondExp} requires four more words to store $i,S_i,N_i,N_{x,i}$. None of the algorithms require more than three counters at once for which we use four words in total. Hence, at most 20 words of memory are required.
%%One word each is required to store $\ell, \bSmp_1, \bSmp_2, \vSmp_1, \vSmp_2$. One word each is required to store $\bar{H}_1, \bar{H}_2,  \widehat{p}_\cA\left(I_1 \right), \widehat{p}_\cA\left(I_2 \right)$ and $\estII$. \textsc{EstProbInt} requires one word to store the counter of the for loop, three words for \textsc{EstInt} and one word for the output of \textsc{EstInt}. Note that once \textsc{EstProbInt} is executed, these words can be freed up for subsequent usage. \textsc{CondExp} uses two words to store $\widehat{H}_i, S_i$ and one word to store $i$. The words freed up after executing  \textsc{EstProbInt} can be used again for the same purpose in \textsc{CondExp}. Finally, one more word is used to store $N_{x,i}$. Therefore, Algorithm~\ref{alg:twoint} uses atmost 20 words.

\medskip
\noindent \textbf{Sample Guarantees.}
%The following theorem establishes sample complexity guarantees on the estimate of Algorithm~\ref{alg:twoint}.
Define Algorithm~\ref{alg:esthi}$^*$ to be a modified version of Algorithm~\ref{alg:esthi} with Step~\ref{step:clip} being 
\[
	\widehat{H}_i = \widehat{H}_i + \log \left(\bSmp_i/(N_{x,i} + 1)\right)
\]
(i.e. without clipping from below) and all other steps remaining the same. Let $\estIIs$ be the output of Algorithm~\ref{alg:twoint} by replacing Step~\ref{step:est_ent} with estimates of Algorithm~\ref{alg:esthi}$^*$. Then we can bound the estimation error by the following three terms and we will bound each of them separately,
\[
	 \left \lvert \Ent{p} -  \estII \right \rvert \le \underbrace{ \left \lvert \Ent{p} -  \Expc{\estIIs} \right \rvert}_\text{Unclipped Bias} + \underbrace{ \left \lvert \Expc{\estII} -  \Expc{\estIIs} \right \rvert}_\text{Clipping Error} + \underbrace{\left \lvert \estII -  \Expc{ \estII}  \right \rvert.
}_\text{Concentration}
\]
%$| \Ent{p} -  \Expc{\estIIs} |$ is the bias of the unclipped algorithm, which is easier to analyze. $| \Expc{\estII} -  \Expc{\estIIs} |$ is the error introduced by the clipping step. And $|\estII -  \Expc{ \estII} |$ can be bounded with high probability because of the nice concentration property of the statistic. Next we will show each of the terms can be bounded by $\eps/3$ if we take the following parameters 
%We show that each of the three terms is bounded above by $\eps/3$.
%\paragraph{Clipping Error.} %We first see how to bound the clipping error term $| \Expc{\estII} -  \Expc{\estIIs} |$ first. 
%By the design of \textsc{CondExp}, we know that $\widehat{H}_2$ is clipped only when the following event occurs for some $x \in \cX$: $ \cE_x= \{ \textsc{EstInt}(\bSmp,x) = I_2, N_{x,2} > 4\bSmp_2 \ell - 1\}$. By Chernoff bound, the probability of $\cE_x$ is very small for values of $\bSmp, \bSmp_2, \ell$ used in Algorithm~\ref{alg:twoint}. Moreover, when the clipping step happens, the error is at most $\log \frac{1}{4\ell}  - \log \left(\frac{\bSmp_2}{\bSmp_2 + 1}\right) \le \log\left( \frac{1}{4\ell}\left(1 + \frac{1}{\bSmp_2}\right) \right) \le \log k$. Hence it suffices to bound $\forall x, \probof{\cE_x} \le \frac{\eps}{3\log k}$. We present the following lemma that bounds the clipping error. (proof in Section~\ref{sec:pfcliptwoint}) 
%\begin{lemma}(\textbf{Clipping Error Bound})\label{lem:cliptwoint}
%Let  $\estII$ be the entropy estimate of Algorithm~\ref{alg:twoint} and let $\estIIs$ be the entropy estimate of the unclipped version of Algorithm~\ref{alg:twoint}. Then 
%$\left \lvert  \Expc{\estII} -  \Expc{\estIIs} \right \rvert \leq {\eps}/{3}.$
%\end{lemma}

\noindent \textbf{Clipping Error.} %We first see how to bound the clipping error term $| \Expc{\estII} -  \Expc{\estIIs} |$ first. 
%By the design of \textsc{CondExp}, we know that $\widehat{H}_2$ is clipped only when the following event occurs for some $x \in \cX$: $ \cE_x= \{ \textsc{EstInt}(\bSmp,x) = I_2, N_{x,2} > 4\bSmp_2 \ell - 1\}$. We can bound the clipping error by showing that $\probof{\cE_x}$ is small. We present the following lemma that bounds the clipping error. (proof in Section~\ref{sec:pfcliptwoint}) 
By the design of \textsc{CondExp}, $\widehat{H}_2$ is clipped only when the event $ \cE_x= \{ \textsc{EstInt}(\bSmp,x) = I_2, N_{x,2} > 4\bSmp_2 \ell - 1\}$ occurs for some $x \in [k]$ . We bound the clipping error in the following lemma (proof in Section~\ref{sec:pfcliptwoint}) by showing that $\probof{\cE_x}$ is small.  
\begin{lemma}(\textbf{Clipping Error Bound})\label{lem:cliptwoint}
	Let  $\estII$ be the entropy estimate of Algorithm~\ref{alg:twoint} and let $\estIIs$ be the entropy estimate of the unclipped version of Algorithm~\ref{alg:twoint}. Then 
	$\left \lvert  \Expc{\estII} -  \Expc{\estIIs} \right \rvert \leq {\eps}/{3}.$
\end{lemma}

%\[
	%\probof{\cE_x} \le \min \{ \probof{EstInt(n,x) = I_2}, \probof{N_{x,2} > 4n_2 \ell - 1}\}
%\]

%By Chernoff bound, if $p(x) > 2 \ell$

%\[ \probof{EstInt(n,x) = I_2} \le \exp\left(-\frac{n \ell}{3}\right)\]

%And if $p(x) < 2 \ell$,

%\[ \probof{N_{x,2} > 4n_2 \ell - 1} \le \exp\left(-\frac{2n_2 \ell}{3}\right)\]

%It is easy to verify that values in~\eqref{eqn:defn} would suffice.
\medskip
\noindent\textbf{Concentration Bound.} To prove the concentration bound, we use Lemma~\ref{lem:concentration} to decompose it into three terms. Each of them can be viewed as the difference between an empirical mean and its true expectation, which can be bounded using concentration inequalities. (proof in Section~\ref{sec:pfconctwoint})

%What remains to be shown is that $|\estII -  \Expc{ \estII} |$ is bounded by $\eps/3$ with probability at least 2/3. First we need the following lemma:

\begin{lemma}(\textbf{Concentration Bound}) \label{lem:concentration}
Let $\estII$ be the entropy estimate of Algorithm~\ref{alg:twoint} and let $\bar{H}_i$ be as defined in Algorithm~\ref{alg:twoint}. Let $p_{\cA}\left(I_i \right)$ be the distribution defined in \eqref{eq:conddist} where $\cA$ is \textsc{EstInt}. Then,
%\vspace{-5pt}
	 \begin{align}
	\left \lvert \Expc{\estII} - \estII \right \rvert \leq \sum\limits_{i=1}^{2}  p_{\cA}\left(I_i\right) \left \lvert \bar{H_i}  - \Expc{\bar{H_i}} \right \rvert + |p_{\cA}\left(I_1\right) - \widehat{p}_{\cA} \left(I_1\right) | |\bar{H}_1 - \bar{H}_2 | \leq {\eps}/{3} \nonumber. 
	\end{align}
\end{lemma}
%Using Lemma~\ref{lem:concentration}, we can decompose the error into three terms and . 




%Moreover, we can bound the concentration error of $\bar{H_1}$ and $\bar{H_2}$ separately by choosing $R_1$ and $R_2$ as we wanted. Next we will try to bound each of the term by $\eps/9$ with high probability.

\newer{We provide a brief outline of the proof below. By the union bound, in order to show that with probability at least $2/3$ the sum is less than $\eps/3$, it is sufficient to show that with probability at most $1/9$, each of the terms is greater than $\eps/9$.

To bound $|p_{\cA}\left(I_1\right) - \widehat{p}_{\cA} \left(I_1\right) | |\bar{H}_1 - \bar{H}_2 |$, we first bound the range of $|\bar{H}_1 - \bar{H}_2 |$ and then use Hoeffding's inequality (Lemma~\ref{lem:hoeff}) to obtain concentration of $\widehat{p}_{\cA} \left(I_1\right)$. To bound  $\left \lvert \bar{H_i}  - \Expc{\bar{H_i}} \right \rvert$, note that we cannot obtain concentration using Hoeffding's inequality because $\vSmp_i$ (the number of samples that we average over) is a random variable. Therefore, we apply Random Hoeffding inequality (Lemma~\ref{lem:ranhoeff}) to $\bar{H_i}$. Since $\vSmp_i$ depends on the range of the random variables being averaged over, we obtain a reduction in the sample complexity for $i=2$ because of clipping the estimate below to $\log \frac{1}{4\ell}$. Therefore, the range for the second interval is $\log(\bSmp_2) - \log \frac{1}{4\ell} = O\left(\log\left( \left(\log k\right)/\eps \right)\right)$ implying $\vSmp_2 = O\left( {(\log \left( (\log  k)/\eps\right))^2}/{\eps^2}\right)$ suffices for the desired probability. For $i=1$, since the range is the same as the one interval case, we use the same $\vSmp_1$ as in the previous section. Note $\vSmp_2 \ll \vSmp_1$.}

\medskip
\noindent\textbf{Bias Bound.} We bound the bias of the unclipped version, $\estIIs$ using the following lemma whose proof is in Section~\ref{sec:pfbiastwo}.

\begin{lemma} (\textbf{Unclipped Bias Bound}) \label{lem:bias_two}
Let $\estIIs$ be the unclipped estimate of Algorithm~\ref{alg:twoint} and let $p_{\cA}\left(I_i \middle| x\right)$ be the conditional distribution defined in \eqref{eq:conddist} where $\cA$ is \textsc{EstProbInt}. Then,
\vspace{-5 pt}
	\begin{align} \label{eq:biastwoint}
	\left| \Ent{p} -  \Expc{\estIIs} \right| \le \sum\limits_{i=1}^{2}  \left( \sum\limits_{x \in \mathcal{X}} { p_{\cA}\left(I_i \middle| x \right)}/{\bSmp_i}\right) \leq {\eps}/{3}.
	\end{align}
\end{lemma}
%\vspace{-5pt}

\newer{Lemma~\ref{lem:bias_two} allows us to choose $\bSmp_1$ and $\bSmp_2$ separately to bound the bias. Interval $I_2$'s contribution is at most $\frac{k}{\bSmp_2}$. For interval $I_1$, we improve upon $\frac{k}{\bSmp_1}$ by partitioning $\cX$ into sets $\cX_1 = \{x \in \cX | p(x) < \ell/2\}$ and $\cX_2  = \{x \in \cX | p(x) \ge \ell/2\}$. For $\cX_1$, $p_{\cA}\left(I_1 \middle| x \right)$ is small by Chernoff bound. For $\cX_2$, since $p(x) \ge \ell/2$, $|\cX_2| \leq 2/\ell$ which is smaller than $k$.  Hence we can choose $N_2 < N_1$.}

In the sample complexity of the two interval algorithm, observe that the term $\bSmp_2\vSmp_2$ dominates. Reducing $\bSmp_2$ is hard because it is independent of the interval length. Therefore we hope to reduce $\vSmp_2$ by partitioning into intervals with smaller lengths. In the smallest interval, if we reduce the range of each estimate to be within a constant, then $O(\frac{1}{\eps^2})$ samples would suffice for concentration. In the next section, we make this concrete by considering an algorithm that uses multiple intervals.
%\vspace{-5 pt}
%\subsection{Two Intervals Algorithm} \label{sec:two_interval}
%We now present some intuition that will be useful to improve the sample complexity of the model algorithm. Let $\ell$ be such that $\frac{1}{k} \leq \ell < \frac{1}{2}$. If we knew beforehand that for some symbols $x$, $p\left(x\right) \geq \ell $, it would be easier to estimate $\log\left(1/p(X)\right)$ since the probability of these symbols is high. In other words, we could use a smaller value of $\bSmp$ for such symbols since their contribution to the bias would be small. On the other hand, for symbols such that $p\left(x\right) \leq \ell $, we could use a smaller value of $\vSmp$ since with high probability, the range of the estimates will be smaller. Therefore, it is possible to reduce the sample complexity further by partitioning symbol probabilities into intervals and using different number of samples to estimate each intervals contribution. \par 
%
%%Lets start by expressing the entropy $\Ent{p}$, in a way that uses the partitions idea explained above. Partition the $\left[0,1 \right]$ interval into $J$ intervals of arbitrary width. Consider an arbitrary conditional distribution $p\left(j \middle| x \right)$ over these intervals given the symbol $x$. We define a marginal distribution over the intervals using this conditional distribution as $p\left[I_j\right] = \sum_{x \in \mathcal{X}} p\left(x\right) p\left( j\middle| x \right)$. The entropy $\Ent{p}$ can be rewritten as follows, 
%%
%%\begin{align}
%% \Ent{p} &= \sum\limits_{x \in \mathcal{X}} p\left(x\right) \log \frac{1}{p\left(x\right)} \nonumber \\
%% &= \sum\limits_{x \in \mathcal{X}} p\left(x\right) \left( \sum\limits_{j=1}^{J} p\left(j \mid x \right) \right) \log \frac{1}{p\left(x\right)} \nonumber \\
%% &=  \sum\limits_{j=1}^{J} \sum\limits_{x \in \mathcal{X}}  p\left(x\right) p\left(j \mid x \right)  \log \frac{1}{p\left(x\right)} \nonumber \\
%% &=  \sum\limits_{j}^{J} p\left[I_j\right]  \sum\limits_{x \in \mathcal{X}}  \frac{p\left(x\right) p\left(j \mid x \right)}{p\left[I_j\right]} \log \frac{1}{p\left(x\right)} \nonumber \\
%% &=  \sum\limits_{j}^{J} p\left[I_j\right] H_j \label{entintexp}
%% \end{align}
%
%In the model algorithm, the key idea was to view $\Ent{p}$ as an expectation of  $\log\left(1/p\left(X\right)\right)$ and estimate the same using an average. In Algorithm~\ref{algentest}, the key idea is to view $\Ent{p}$ as the product $p\left[I_j\right] H_j $  over all the intervals. Additionally, $H_j$ can be viewed as a conditional expectation of $\log\left(1/p\left(X\right)\right)$ with respect to the conditional distribution $p\left(x \middle| j \right) = \frac{p\left(x\right) p\left(j \mid x \right)}{p\left[I_j\right]}$. As in the model algorithm, Algorithm~\ref{algentest} estimates this conditional expectation $H_j$, using an average. Algorithm~\ref{algintvlesti} estimates $p\left[I_j\right]$ independently of $H_j$. \par
%
%We will now specify the details of Algorithm~\ref{algentest} and Algorithm~\ref{algintvlesti}. We consider a partition of the $\left[0,1\right]$ interval into two intervals defined as follows : 
%\begin{equation}
%I_2 = \left[0,\ell \right], I_1 = \left[\ell,1\right] \hspace{5mm} \text{where} \hspace{5mm} \ell = \frac{\left(\log k \right)^{\beta}}{k}.
%\end{equation}
%
% Algorithm~\ref{algintvlesti} generates a sample $X \sim p$ and outputs an interval in which $p\left(X\right)$ is likely to lie in. Conditioned on the event that symbol $x$ was sampled in line 2 of Algorithm~\ref{algintvlesti}, a conditional probability distribution can be defined over the intervals,  $p\left(i \middle| x\right) = \Pr\left(\text{EstInt} = I_i \middle| x \right)$. Using this conditional distribution, a marginal distribution $p\left[I_i\right] = \sum_{x \in \mathcal{X}} p\left(x\right) p\left(i\middle| x\right) $ can be defined over the intervals. \par 
%
% 
%Algorithm~\ref{algentest} uses Algorithm~\ref{algintvlesti} as a subroutine to estimate $p\left[I_j\right]$. Note that it is sufficient to estimate $p\left[I_1\right]$ since $p\left[I_2\right] = 1 - p\left[I_1\right]$. Independent of $p\left[I_j\right]$'s, Algorithm~\ref{algentest} estimates the conditional expectation $H_j$ for each interval $I_j$ as an average over $R_j$ samples. Since the average is over the conditional distribution $p\left(x \middle| j \right)$, Algorithm~\ref{algintvlesti} is called again. If the output of Algorithm~\ref{algintvlesti} matches the interval under consideration, $\log\left(1/p\left(X\right) \right)$ is estimated as in the model algorithm.
% We fix the parameters used in the algorithm in terms of constants $C_1,C_2, \gamma < \beta $. \todo{No values to the constants}
%\begin{align}
%n_2 &= C_1 \cdot \frac{k}{\eps}, \hspace{5mm} n_1 = C_1 \cdot\frac{k}{\eps \left( \log k \right)^{\gamma} }.\\
%R_2 &= C_2 \cdot \frac{\left(\log \log k\right)^2}{\epsilon^2}, \hspace{5mm} R_1 = C_2 \frac{\log^2 k}{\eps^2}.
%\end{align}
% 
%\begin{algorithm}[H]
%\caption{Entropy estimation : Two Intervals Algorithm} \label{algentest}
%\begin{algorithmic}[1]
%\State $\widehat{p}\left[I_1\right], \widehat{p}\left[I_2\right] = 0$
%\For{$t = 1 \text{ to } R_1$}
%	\State Output = $\text{EstInt}\left(n_1\right)$
%	\If{Output is $I_1$}
%		\State $\widehat{p}\left[I_1\right] = \widehat{p}\left[I_1\right] + \frac{1}{R_1}$
%	\EndIf
%\EndFor
%\For{$i=1,2$}
%	\State $\widehat{H}_i = 0, S_i = 0$
%	\For{$t=1 \text{ to } R_i$}
%		\State Output =   $\text{EstInt}\left(n_i\right)$ and let $x$ be the sample generated in Algorithm~\ref{algintvlesti}
%		\If{Output is $I_i$}
%			\State $S_i = S_i + 1$
%			\State Sample $n_i$ more samples from $p$ \label{computehl1}
%			\State Let $N_{x,i}$ be the number of times $x$ appears in the $n_i$ samples \label{computehl2}
%			\State $\widehat{H}_i = \widehat{H}_i + \log \left(\dfrac{n_i}{N_{x,i} + 1} \right)$
%		\EndIf
%	\EndFor
%	\State $\widehat{H}_i = \dfrac{\widehat{H}_i}{S_i}$
%\EndFor
%\State Output  $\widehat{H} = \widehat{p}\left[I_1\right] \widehat{H_1} + \left(1-\widehat{p}\left[I_1\right]\right) \widehat{H_2}$
%\end{algorithmic}
%\end{algorithm} 
%
%\begin{theorem}\label{thm:twoint}
%The entropy estimate of Algorithm~\ref{algentest} uses $O\left(1\right)$ words and its sample complexity satisfies 
%\begin{equation}
% \SamC{k}{\epsilon}{\frac{1}{4}} = O\left(\dfrac{k \left( \log \log k\right)^2}{\eps^3}\right).
% \end{equation}
%\end{theorem} 
%\begin{proof}
% Since, Algorithm~\ref{algentest} does not store more than two samples at an instance, it uses $O\left(1\right)$ words of memory. Given the values of $n_1,n_2,R_1,R_2$, the number of samples used by  Algorithm~\ref{algentest} is $O\left( n_1R_1 + n_2R_2 \right) = O\left(\dfrac{k \left( \log \log k\right)^2}{\eps^3}\right) $. \par 
%Finally, to prove that with probability atleast $\frac{3}{4}$, $\left \lvert \widehat{H} - H\left(p\right) \right \rvert \leq \eps$, we use the following two lemmas whose proofs are deferred to Section~\ref{sec:twointproofs}
%
%\begin{lemma}(\textbf{Bias bound})\label{lem:twobias}
%For the entropy estimate $\widehat{H}$ of Algorithm~\ref{algentest}, 
%\begin{equation*}
%\left \lvert \Ent{p} - \Expc{\widehat{H}} \right \rvert \leq \frac{\epsilon}{2}.
% \end{equation*}
%\end{lemma}  
%
%\begin{lemma}(\textbf{Concentration bound})\label{lem:twovar}
%For the entropy estimate $\widehat{H}$ of Algorithm~\ref{algentest}, 
%\begin{equation*}
%\Pr \left(\left \lvert \widehat{H} - \Expc{\widehat{H}} \right \rvert > \frac{\epsilon}{2} \right) \leq \frac{1}{4} .
%\end{equation*}
%\end{lemma}
%
%\end{proof}
%
% 
% 
% 
 
